SDN-Assisted Network-Based Mitigation of Slow DDoS Attacks

Slow-running attacks against network applications are often not easy to detect, as the attackers behave according to the specification. The servers of many network applications are not prepared for such attacks, either due to missing countermeasures or because their default configurations ignores such attacks. The pressure to secure network services against such attacks is shifting more and more from the service operators to the network operators of the servers under attack. Recent technologies such as software-defined networking offer the flexibility and extensibility to analyze and influence network flows without the assistance of the target operator. Based on our previous work on a network-based mitigation, we have extended a framework to detect and mitigate slow-running DDoS attacks within the network infrastructure, but without requiring access to servers under attack. We developed and evaluated several identification schemes to identify attackers in the network solely based on network traffic information. We showed that by measuring the packet rate and the uniformity of the packet distances, a reliable identificator can be built, given a training period of the deployment network.

==> chapters/outlook.tex <==
% Length: (Outlook & Conclusion) 1.25
% Responsible: T

%\section{Outlook}
%\label{sec:outlook}

eierlegendewollmilchsau
\todo[inline]{Responsible: T}

\todo[inline]{(be) practical implications: Was bedeuten unsere Ergebnisse für die Community? Für ISPs, die sowas umsetzen wollen? Was davon ist verallgemeinerbar?}
wird möglich slow based angriffe abzuwehren ohne dass kunden eingreifen müssen (services anpassen müssen)
thresholds sind netzwerkspezifisch

\todo[inline]{(be) Outlook: was sind generelle, noch offene Forschungsfragen (unabhängig von unserer Agenda)}
machine learning auf dem ding?


wie kommt man mit wenig aufwand zu thresholds?

